Parrot: Efficient Serving of LLM-based Applications with Semantic Variable

The rise of large language models (LLMs) has enabled LLM-based applications (a.k.a. AI agents or co-pilots), a new software paradigm that combines the strength of LLM and conventional software. Diverse LLM applications from different tenants could design complex workflows using multiple LLM requests to accomplish one task. However, they have to use the over-simplified request-level API provided by today's public LLM services, losing essential application-level information. Public LLM services have to blindly optimize individual LLM requests, leading to sub-optimal end-to-end performance of LLM applications. This paper introduces Parrot, an LLM service system that focuses on the end-to-end experience of LLM-based applications. Parrot proposes Semantic Variable, a unified abstraction to expose application-level knowledge to public LLM services. A Semantic Variable annotates an input/output variable in the prompt of a request, and creates the data pipeline when connecting multiple LLM requests, providing a natural way to program LLM applications. Exposing Semantic Variables to the public LLM service allows it to perform conventional data flow analysis to uncover the correlation across multiple LLM requests. This correlation opens a brand-new optimization space for the end-to-end performance of LLM-based applications. Extensive evaluations demonstrate that Parrot can achieve up to an order-of-magnitude improvement for popular and practical use cases of LLM applications.

==> deprecated/1-intro.tex <==
\section{Introduction}
The emergence of large language models (LLMs) is changing the paradigm of how new applications are built. 
A new paradigm called AI agent (or Co-pilot) has been proposed to enhance the capability of traditional programming language with \emph{semantic programming}, i.e., expressing the semantic/intention of a function using natural language and using LLM to generate the output. These LLM-executed functions are called \emph{semantic functions} in the rest of this paper.
Many tools have been proposed for developing AI agents (or co-pilots), e.g., Langchain~\cite{}, Semantic Kernel~\cite{}, to build AI agents with \emph{semantic functions}.%, that combine intelligence from LLMs (using natural language) with conventional programming language. A semantic function can be abstracted as a function whose input and output are texts, and it is executed by inference of an LLM. 
An AI agent application usually comprises multiple semantic functions that work collaboratively to complete one universal goal. For example, MetaGPT~\cite{} introduces multiple roles like project managers, architects, and programmers to communicate with each other to develop a code project. AutoGen~\cite{} allows customization of multi-agent conversations. This new application paradigm not only lowers the burden of programming but also brings many new capabilities empowered by LLMs. It is likely to be a vital and growing workload, especially in cloud data centers.

A high-quality AI agent application is unlikely composed of a single semantic function. It is important for semantic functions to interact to accomplish a complex task. However, existing LLM service providers (e.g., OpenAI, Azure, Claude) support AI agent applications in a very primitive way. They provide a text completion API which an application provides a text prompt, and the LLM service responds with the generated text. The interaction of semantic functions is totally accomplished by clients (native code of AI agent), incurring heavy message forwarding and re-scheduling overhead (30~60\% of API time in our production measurement). Moreover, by analyzing the popular AI agents in our production and the open-source community, we identify many optimization opportunities by exploiting the interactions and correlations of different semantic functions, which are impossible for existing single-request-centric LLM services. %, e.g., pipelined communication of the output of a semantic function to the inputs of semantic functions avoiding the forwarding overhead.

%Unfortunately, it is difficult for existing LLM services to exploit such opportunities because of the hardness of understanding the correlations among semantic functions. 
The hardness of understanding the correlations among semantic functions is the root cause of why existing LLM services are inefficient when serving AI agent applications. AI agent developers usually design different text regions with different semantic purposes in one semantic function, e.g., task instruction, few-shot examples, input data, and output data. However, with the existing text completion API, such information is buried under the pure text data without any differentiation of semantics. When multiple LLM inference requests share the same text region or communicate with each other using specific text regions, the LLM service can hardly identify such correlations in an online manner.

In this paper, we propose \sysname{}, a cloud-scale LLM service system that treats AI agents as first-class citizens. \sysname{} unifies the expression of semantic functions using \sv{} to annotate text regions with different semantic purposes for ease of analysis. %At the core of \sysname{} is the data abstraction called \sv{} that lets AI agent developers annotate the semantic granularity of texts in semantic functions. 
By tracing \sv{}s in semantic functions, \sysname{} can easily understand more fine-grained similarity and dependency of semantic functions, bringing a new optimization space. 

First of all, multiple semantic functions can be connected using the same \sv{} to realize inter-function communication on the fly. When these semantic functions are submitted to cloud LLM service, the \sv{} generated by one semantic function will be transferred, and computed to the input of subsequent semantic functions in a pipelined manner, bypassing the heavy overhead of client-side forwarding. %tokenization/detokenization, format parsing, network, and rescheduling overhead. 
\sysname{} can further dissect the dependency of semantic functions into the \sv{}-level, allowing simultaneous and asynchronous execution of \sv{}s for lower end-to-end latency. Also, \sysname{} can easily extract the common \sv{} across semantic functions in an online manner, whose computation and storage can be de-duplicated. 

To support a cloud-scale LLM service, \sysname{} will receive requests from diverse AI agent applications with different performance objectives. \sysname{} can derive the scheduling preference (latency vs. throughput) of each semantic function in order to optimize the end-to-end performance of an application. %\sysname{} can schedule semantic functions to optimize their end-to-end application performance. 
For example, a latency-sensitive application may need to maximize the throughput of certain semantic functions for optimal latency, instead of optimizing the latency of individual requests.

We extensively evaluate \sysname{} on popular AI agents, including our production applications and open-sourced projects, on a cluster of 64 GPUs. With the proposed multi-request optimizations, our evaluation shows \sysname{} achieves up to xx speedup (xx on average) compared with the state-of-the-art solutions. The key contributions are as follows:
\begin{itemize}[leftmargin=*]
\item We identify the misalignment between existing request-centric LLM services and AI agent applications, the root cause of inefficient serving.
\item We identify a new optimization space for serving AI agents by understanding fine-grained \sv{}-level dependency.
\item We propose the \sv{} abstraction to unify the expression of semantic functions, making their dependency easy to analyze.
\item We propose multiple optimizations for serving AI agents by exploiting the \sv{}-dependency analysis, which is shown effective for popular AI agent applications.
\end{itemize}

%By analyzing their semantic-level correlations, we propose xxx optimizations: (1) asynchronously executing semantic functions at the granularity of \sv{}; (2) pipelined communication of \sv{} on the fly; (2)


%schedule requests with the same optimization objective (e.g., OpenAI optimizes for latency)

==> deprecated/5-eval.tex <==
\section{Evaluation}

% \begin{table*}[h]
%     \caption{Scenarios used for evaluation}
%     \label{tab:experiments}
%     \centering
%     \footnotesize
%     \begin{tabularx}{0.9\textwidth}{|c|c|c|c|c|c|}
%     \hline
%     ~ & ~ & IRC & Diverse Req Spec & Diverse App Spec & Shared Prompt & Fine-Grained Parallel\\
%     \hline
%     Data Analytics & Meeting Note Generation (chain) & $\checkmark$ &  &  &  & $\checkmark$\\
%      & Document Summary (map-reduce) & ~ & $\checkmark$ &  &  & \\
%     \hline
%     Long-System Prompt & Bing Copilot (Syndey) response / GPTs & ~ &  &  & $\checkmark$ & \\
%     \hline
%     Multi-Agent System & MetaGPT & $\checkmark$ & $\checkmark$ &  & $\checkmark$ & \\
%     \hline
%     Mixed Workload & from above all~ & ~ & ~ & $\checkmark$ & ~ & ~ \\
%     \hline
%     \end{tabularx}
% \end{table*}

\subsection{Experimental Setup}
\paragraph{Testbed.}

\paragraph{Benchmarks and datasets.}

\paragraph{Baselines.}

\subsection{Micro-benchmarks}
\paragraph{Latency reduction by avoiding local forwarding.}
    \begin{itemize}
        \item Workload: Multiple ReAct Applications (e.g., AutoGen?) co-run in a shared GPU cluster
        \item 4*A6000
        \item Baseline: Round-robin, client-side forwarding
        \item Ours: app-level round-robin, semantic functions from the same app will be scheduled at the same GPU.
    \end{itemize}

\paragraph{Derive request performance from e2e app performance objective}
    \begin{itemize}
        \item Workload: MapReduce Summarization + Chat
        \item 4*A6000
        \item Baseline: BS=4,16
        \item Ours: BS=16 for map tasks, BS=4 for chat and reduce
    \end{itemize}
    
\paragraph{Shared Prompt in the same session and across sessions} 
    \begin{itemize}
        \item Workload: Bing Chat, AutoGen
        \item 4*A6000
        \item Baseline: BS=4
        \item Ours: Share Prompt BS=? Same per token latency, compare throughput.
    \end{itemize}
    
\paragraph{Async execution} (TBD, low gain due to generation-dominated)
    \begin{itemize}
        \item Workload: Chain-summarization
        \item A100
        \item Baseline: BS=4
        \item Ours: Async execution+concat online
    \end{itemize}
\subsection{End-to-end Evaluation}
    \begin{itemize}
        \item A mixture of all the above workloads
        \item 64*V100
        \item Baseline: BS=4 + Request-level Round-robin
        \item Ours: Share prompt + Adaptive BS + App-level Round-robin
    \end{itemize}
